Generative Autoregressive Transformers for Model-Agnostic Federated MRI Reconstruction

While learning-based models hold great promise for MRI reconstruction, single-site models trained on limited local datasets often show poor generalization. This has motivated collaborative training across institutions via federated learning (FL)-a privacy-preserving framework that aggregates model updates instead of sharing raw data. Conventional FL requires architectural homogeneity, restricting sites from using models tailored to their resources or needs. To address this limitation, we propose FedGAT, a model-agnostic FL technique that first collaboratively trains a global generative prior for MR images, adapted from a natural image foundation model composed of a variational autoencoder (VAE) and a transformer that generates images via spatial-scale autoregression. We fine-tune the transformer module after injecting it with a lightweight site-specific prompting mechanism, keeping the VAE frozen, to efficiently adapt the model to multi-site MRI data. In a second tier, each site independently trains its preferred reconstruction model by augmenting local data with synthetic MRI data from other sites, generated by site-prompting the tuned prior. This decentralized augmentation improves generalization while preserving privacy. Experiments on multi-institutional datasets show that FedGAT outperforms state-of-the-art FL baselines in both within- and cross-site reconstruction performance under model-heterogeneous settings.

==> tables/selffid.tex <==
% Calculating self-FID (10% vs 90%) for real data: fastmri_knee ...
% Calculating self-FID (10% vs 90%) for real data: fastmri_knee ...

% fastmri_knee self-FID: 0.07  [10th: 0.03, 90th: 0.14]

% Calculating self-FID (10% vs 90%) for real data: fastbrain ...
% fastbrain self-FID: 0.07  [10th: 0.02, 90th: 0.14]

% Calculating self-FID (10% vs 90%) for real data: umram ...
% umram self-FID: 0.01  [10th: 0.00, 90th: 0.01]

% Calculating cross-FID (10% GAT vs full real) for: fastmri_knee ...
% fastmri_knee_vat cross-FID: 0.66  [10th: 0.58, 90th: 0.73]

% Calculating cross-FID (10% GAT vs full real) for: fastbrain ...
% fastbrain_vat cross-FID: 0.53  [10th: 0.49, 90th: 0.59]

% Calculating cross-FID (10% GAT vs full real) for: umram ...
% umram_vat cross-FID: 0.07  [10th: 0.06, 90th: 0.08]
